On the Nature and Genesis of EUV Waves: A Synthesis of Observations from SOHO, STEREO, SDO, and Hinode

A major, albeit serendipitous, discovery of the SOlar and Heliospheric Observatory mission was the observation by the Extreme Ultraviolet Telescope (EIT) of large-scale Extreme Ultraviolet (EUV) intensity fronts propagating over a significant fraction of the Sun's surface. These so-called EIT or EUV waves are associated with eruptive phenomena and have been studied intensely. However, their wave nature has been challenged by non-wave (or pseudo-wave) interpretations and the subject remains under debate. A string of recent solar missions has provided a wealth of detailed EUV observations of these waves bringing us closer to resolving their nature. With this review, we gather the current state-of-art knowledge in the field and synthesize it into a picture of an EUV wave driven by the lateral expansion of the CME. This picture can account for both wave and pseudo-wave interpretations of the observations, thus resolving the controversy over the nature of EUV waves to a large degree but not completely. We close with a discussion of several remaining open questions in the field of EUV waves research.

==> referee_report <==
Minor issues:

Sect. 1, end of para. 6:
"The two fronts exist, ..."

Sect. 11, page 30:
Figure 21 is not correctly referenced in the main text, it says "Figure ??"
-----










The only scientific question I have is related to Eq. (1):
shouldn't that be the group velocity instead of the phase velocity? Are they
identical? Even if they are, I think the correct variable here is the v_gr,
not v_ph.

"Reproduced by permission of the AAS".
Credit: Author, A&A, vol, page, year, reproduced with permission \copyright ESO.


Some typos:

- p.5 l.25: "the genesis of EUV waves and theN describe"

- p.6 l.9,10: references should be in brackets

- p 8 l.33,34: references should be in brackets

- p 11 l.39: reference (Olemdo ..) should be in brackets

- p 12 l.33: reference (Veronig ..) should be in brackets

-p 12 l.42: of the event of the 2010 June 13  (one "the" too many)

-p 13 l.13: reference Hershaw should be in brackets

-p 13 l.19: velocities (instead of velocityies)

-p 17 l.34: CAME I guess should be CME

-p 20 l39,40: Wamuth and Vrsnak below should be in parenthesis

-p 22 l.50: Lui et al should be in parenthesis

-p 23 l41: He II (instead of HeII)

-p 30 l42: Figure ??

- p31 l45: blank missing before Figure 19

- p37 l21: period after (see Figure 7) missing
-----

